Laboratory Investigations of Titan Haze Formation: In Situ Measurement of Gas and Particle Composition

Prior to the arrival of Cassini-Huygens, aerosol production in Titan's atmosphere was believed to begin in the stratosphere where chemical processes are predominantly initiated by FUV radiation. However, measurements taken by Cassini UVIS and CAPS indicate that haze formation initiates in the thermosphere where there is a greater flux of EUV photons and energetic particles available to initiate chemical reactions, including the destruction of N2. The discovery of previously unpredicted nitrogen species in Titan's atmosphere by Cassini INMS indicates that nitrogen participates in the chemistry to a much greater extent than was appreciated before Cassini. The degree of nitrogen in the haze is important for understanding the diversity of molecules present in Titan's atmosphere and on its surface. We have conducted a series of simulation experiments using either spark discharge or FUV photons to initiate chemistry in CH4/N2 gas mixtures (0.01% CH4/99.99% N2 to 10% CH4/90% N2). We obtained in situ real-time measurements using an HR-ToF-AMS to measure the particle composition as a function of particle size and a PIT-MS to measure the composition of gas phase products. These two techniques allow us to investigate the effect of energy source and initial CH4 concentration on the degree of nitrogen incorporation in both the gas and solid phase products. The results presented here confirm that FUV photons produce not only solid phase nitrogen bearing products but also gas phase nitrogen species. We find that in both the gas and solid phase, nitrogen is found in nitriles rather than amines and both the gas phase and solid phase products are composed primarily of molecules with a low degree of aromaticity. The UV experiments reproduce the absolute abundances measured in Titan's stratosphere for a number of gas phase species including C4H2, C6H6, HCN, CH3CN, HC3N, and C2H5CN. [Edited for length]

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

